CLIP meets DINO for Tuning Zero-Shot Classifier using Unlabeled Image Collections

In the era of foundation models, CLIP has emerged as a powerful tool for aligning text & visual modalities into a common embedding space. However, the alignment objective used to train CLIP often results in subpar visual features for fine-grained tasks. In contrast, SSL-pretrained models like DINO excel at extracting rich visual features due to their specialized training paradigm. Yet, these SSL models require an additional supervised linear probing step, which relies on fully labeled data which is often expensive and difficult to obtain at scale. In this paper, we propose a label-free prompt-tuning method that leverages the rich visual features of self-supervised learning models (DINO) and the broad textual knowledge of large language models (LLMs) to largely enhance CLIP-based image classification performance using unlabeled images. Our approach unfolds in three key steps: (1) We generate robust textual feature embeddings that more accurately represent object classes by leveraging class-specific descriptions from LLMs, enabling more effective zero-shot classification compared to CLIP's default name-specific prompts. (2) These textual embeddings are then used to produce pseudo-labels to train an alignment module that integrates the complementary strengths of LLM description-based textual embeddings & DINO's visual features. (3) Finally, we prompt-tune CLIP's vision encoder through DINO-assisted supervision using the trained alignment module. This three-step process allows us to harness the best of visual & textual foundation models, resulting in a powerful and efficient approach that surpasses state-of-the-art label-free classification methods. Notably, our framework, NoLA (No Labels Attached), achieves an average absolute gain of 3.6% over the state-of-the-art LaFTer across 11 diverse image classification datasets. Our code & models can be found at https://github.com/fazliimam/NoLA.

==> tables/ablation_table_CDEvDL.tex <==
\begin{table}[H]
    \caption{\textnormal{\textbf{Ablation of using the CDE classifier as the pseudo-labeller in the FixMatch part compared against using DINO backbone.} The top-1 accuracy for each variant is averaged across six datasets for their respective test sets.}}
    \centering
    \begin{tabular}{l c}
    \toprule
      & Top-1 Acc. \\
    \midrule
     $\text{NoLA}^{\dagger}$ & {76.18} \\
    NoLA & 80.5 \\
    \bottomrule
    \end{tabular}
    \label{tab:ablation3}
\end{table}


==> tables/ablation_table_clipvdino.tex <==
\begin{table}[H]
    \caption{\textnormal{\textbf{Ablation of using CLIP backbone in the DL network compared against using pre-trained DINO backbone.} The top-1 accuracy for each variant is averaged across six datasets for their respective test sets.}}
    \centering
    \begin{tabular}{l c}
    \toprule
     Backbone & Top-1 Acc. \\
    \midrule
    CLIP & 77.8 \\
    DINO & 80.5 \\
    \bottomrule
    \end{tabular}
    \label{tab:ablation3}
\end{table}


==> tables/suppl_4.tex <==
% FOR SUPPLEMENTARY

\begin{table}[H]
\setlength{\tabcolsep}{4pt}
    \centering % Center the table
    \caption{\textnormal{\textbf{.}}}
    \small % Adjust font size here
    \begin{tabular}{lccccccc}
    \toprule
     & \rotatebox{90}{EuroSAT} & \rotatebox{90}{Caltech101} & \rotatebox{90}{Oxford-Pets} & \rotatebox{90}{Flowers-102} & \rotatebox{90}{SUN397} & \rotatebox{90}{CIFAR100} \\
    \midrule
    # of training images  \\
    # of classes \\
    Avg. # of images per class \\
    Proportion \\
    k \\
    \bottomrule
    \end{tabular}
    \label{tab:suppl4}
\end{table}

